Conservative Contextual Bandits: Beyond Linear Representations

Conservative Contextual Bandits (CCBs) address safety in sequential decision making by requiring that an agent's policy, along with minimizing regret, also satisfies a safety constraint: the performance is not worse than a baseline policy (e.g., the policy that the company has in production) by more than $(1+\alpha)$ factor. Prior work developed UCB-style algorithms in the multi-armed [Wu et al., 2016] and contextual linear [Kazerouni et al., 2017] settings. However, in practice the cost of the arms is often a non-linear function, and therefore existing UCB algorithms are ineffective in such settings. In this paper, we consider CCBs beyond the linear case and develop two algorithms $\mathtt{C-SquareCB}$ and $\mathtt{C-FastCB}$, using Inverse Gap Weighting (IGW) based exploration and an online regression oracle. We show that the safety constraint is satisfied with high probability and that the regret of $\mathtt{C-SquareCB}$ is sub-linear in horizon $T$, while the regret of $\mathtt{C-FastCB}$ is first-order and is sub-linear in $L^*$, the cumulative loss of the optimal policy. Subsequently, we use a neural network for function approximation and online gradient descent as the regression oracle to provide $\tilde{O}(\sqrt{KT} + K/\alpha) $ and $\tilde{O}(\sqrt{KL^*} + K (1 + 1/\alpha))$ regret bounds, respectively. Finally, we demonstrate the efficacy of our algorithms on real-world data and show that they significantly outperform the existing baseline while maintaining the performance guarantee.

==> sec/unknown_baseline.tex <==
In this section we relax the the assumption of knowing the true baseline cost values to having an un-biased
estimate of the baseline cost. More formally, consider the following filtration
\begin{align*}
    \cF_{t-1} = \sigma \bigg((\x_{i,a},{a}_i,y_{i,\tilde{a}_i}), \x_{t,a}; 1 \leq i \leq t-1, a \in [K] \bigg).
\end{align*} 
Then we assume that we have good estimates $\hat{h}(\x_{t,b_t})$ of the baseline costs, i.e.,
\begin{align*}
    \E[\hat{h}(\x_{t,b_t}) | \cF_{t-1}] = h(\x_{t,b_t}), \;\; \forall t\in [T]
\end{align*}
We can slightly modify our algorithms to retain the same regret bound and performance constraint guarantees. 
Consider $\cSquareCB$ (Algorithm~\ref{algo:C-SquareCB}) and replace the \emph{safety condition} in \eqref{eq:safety-condition} by the following more stringent condition:
% \begin{align}
%     & \underbrace{\hat{y}_{t, \Tilde{a}_{t}} + \underset{i\in \cS_{t-1}}{\sum}\underset{a\in[K]}{\sum}p_{i,a}\hat{y}_{i, a}}_{(A)} +  \underbrace{\underset{i\in \cS^c_{t-1}}{\sum}\hat{h}(\x_{i,b_i})}_{(B)} + \underbrace{16 \sqrt{m_{t-1} \bigg(\regsq(m_{t-1}) + \log(4/\delta)\bigg)}}_{(C)} \nonumber \\
%     & \qquad\qquad \underbrace{2 \sqrt{n_{t-1}\log(2\delta^{-1})}}_{(D)} \;\; \leq \;\;  (1+\alpha)\overset{t}{\underset{i=1}{\sum}}\;\;\hat{h}(\x_{i,b_t}) - \underbrace{2 \sqrt{t\log(2\delta^{-1})}}_{(E)}.
%     \label{eq:safety-condition}
% \end{align}
\begin{align}
    & \underbrace{\hat{y}_{t, \Tilde{a}_{t}} + \underset{i\in \cS_{t-1}}{\sum}\underset{a\in[K]}{\sum}p_{i,a}\hat{y}_{i, a}}_{(A)}  + \underbrace{16 \sqrt{m_{t-1} \bigg(\regsq(m_{t-1}) + \log(4/\delta)\bigg)}}_{(C)} - \alpha \nonumber \\
    & \qquad\qquad  \;\; \leq \;\;  (1+\alpha){\underset{i \in \cS_{t-1}}{\sum}}\;\;\hat{h}(\x_{i,b_t}) - \underbrace{2 \sqrt{m_{t}\log(2\delta^{-1})}}_{(D)}.
    \label{eq:safety-condition2}
\end{align}
\begin{align}
    \underbrace{\hat{y}_{t, \Tilde{a}_{t}} + \underset{i\in \cS_{t-1}}{\sum}\underset{a\in[K]}{\sum}p_{i,a}\hat{y}_{i, a}}_{(A)} +  \underbrace{\underset{i\in \cS^c_{t-1}}{\sum}h(\x_{i,b_i})}_{(B)} & + \underbrace{16 \sqrt{m_{t-1} \bigg(\regsq(m_{t-1}) + \log(4/\delta)\bigg)}}_{(C)} \nonumber \\
    & \leq  (1+\alpha)\overset{t}{\underset{i=1}{\sum}}\;\;h(\x_{i,b_i}).
    \label{eq:safety-condition}
\end{align}
where recall that $n_t = |\cS_t^c|$. Note that term $(A)$ remains same as before, we removed term $(B)$ from \eqref{eq:safety-condition} and term $(C)$ is as before. In the rhs, we changed the sum from $i \in [T]$ in \eqref{eq:safety-condition} to $i \in \cS_{t-1}$ in \eqref{eq:safety-condition2}, and replaced $h$ by its estimate $\hat{h}$. Finally we introduced a new term $(D)$. Term $(D)$ is essentially the Hoeffding buffer and ensures that the algorithm is conservative enough even with the estimates $\hat{h}$. 


and therefore using Azuma-Hoeffding we have that with probability $\displaystyle 1-\delta$
    \begin{align}
    \label{eq:performance-term-II}
        \Bigg| \sum_{i \in \cS_{t-1}} \sum_{a \in [K]} p_{i,a} h(\x_{i,a}) - h(\x_{i,\tilde{a}_i})\Bigg| \leq 2 \sqrt{m_{t-1}\log(2\delta^{-1})}
    \end{align}
